Microscale 3-D Capacitance Tomography with a CMOS Sensor Array

Electrical capacitance tomography (ECT) is a nonoptical imaging technique in which a map of the interior permittivity of a volume is estimated by making capacitance measurements at its boundary and solving an inverse problem. While previous ECT demonstrations have often been at centimeter scales, ECT is not limited to macroscopic systems. In this paper, we demonstrate ECT imaging of polymer microspheres and bacterial biofilms using a CMOS microelectrode array, achieving spatial resolution of 10 microns. Additionally, we propose a deep learning architecture and an improved multi-objective training scheme for reconstructing out-of-plane permittivity maps from the sensor measurements. Experimental results show that the proposed approach is able to resolve microscopic 3-D structures, achieving 91.5% prediction accuracy on the microsphere dataset and 82.7% on the biofilm dataset, including an average of 4.6% improvement over baseline computational methods.

==> plots/experimental_plot.tex <==
\begin{figure}[!h]
    \centering

    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]
    {figures/exp_setup/sensor2.pdf}
    \vspace*{-2mm}
    \captionsetup{font={small}}
    \caption{}
    \end{subfigure}   \smallskip
    

    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/exp_setup/ect_image_plot_scalebar.pdf}
    \includegraphics[width=0.3\textwidth]{figures/exp_setup/conf_image_plot2_scalebar.pdf}
    \vspace*{-2mm}
    \captionsetup{font={small}}
    \caption{}
    \end{subfigure}
    \captionsetup{font={small}}
    \caption{(a) The CMOS microelectrode array has 131,072 electrodes on a 10 micron grid. (b) Experimental samples were mounted to allow both ECT measurements as well as 3-D optical images from a confocal microscope. (b) An example dataset acquired with a \emph{B. subtilis} biofilm showing the confocal max projection (right) and the ECT image (left). \JKR{Expand the microscope cross-section, increase text size, include more about the microscope (still simplified of course).} \JKR{Please do not squash graphics aspect ratios.}}%
    \vspace*{-6mm}
    \label{fig:exp_setup}
\end{figure}

==> tables/sota_table_big.tex <==

\begin{table*}[h]

\centering
\caption{\label{ablation} Qualitative comparison to prior work}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{c | c | l | l | l | l| l| l | l} 
 \hlineB{2.5}
  & Dataset & MSE \downarrow &  MAE \downarrow  & SSIM \uparrow & PSNR \uparrow & CC \uparrow & IoU \uparrow  & MPA \uparrow \\ [0.5ex] 
 \hlineB{2.5}
 \multirow{2}[]{9em}{Tikhonov} 
& $\Omega_1$ & -- & -- & -- & -- & -- & -- & -- \\ 
& $\Omega_2$ & -- & -- & -- & -- & -- & --  & --\\ [0.5ex] 
 \hline

\multirow{2}[]{9em}{FNN-AE \cite{Zheng}} 
& $\Omega_1$ & 0.0252 & 0.6936 & 15.9889 & 0.3448 & 0.4853 & -- & --\\ 
& $\Omega_2$ & 0.1459 & 0.6787 & 8.3607 & 0.4475 &  0.5917 & -- & --\\ [0.5ex] 
 \hline

\multirow{2}[]{9em}{FNN+CNN-AE \cite{Zhu}} 
& $\Omega_1$ & 0.0206  & 0.9252 & 16.8668 & 0.6868 & 0.7499 & -- & --\\ 
& $\Omega_2$ & 0.1246 & 0.6569 & 9.0435 & 0.6157 &  0.6854 & -- & -- \\ [0.5ex] 
 \hline

\multirow{2}[]{9em}{Self-attention+UNet \cite{transformer}} 
& $\Omega_1$ & -- & -- & -- & -- & -- & -- & --\\ 
& $\Omega_2$ & -- & -- & -- & -- & --  & -- & --\\ [0.5ex] 
 \hline
 
\multirow{2}[]{9em}{TCNN+MOL (Ours)} 
& $\Omega_1$  & \textbf{0.0147} & \textbf{0.9423} & \textbf{18.32} & \textbf{0.75} &  \textbf{0.79} & -- & --\\ 
& $\Omega_2$ & \textbf{0.0625}  & \textbf{0.7886} & \textbf{12.040} & \textbf{0.810} & \textbf{0.7641} & --  & --\\ [0.5ex] 

 \hlineB{2.5}

 \hline
 
\end{tabular}
% }
\end{table*}



